Testing time evolution of the mass distribution of the black hole mergers

The detection of gravitational-wave events revealed that there are numerous populations of black hole (BH) binaries that can merge within the age of the Universe. Although several formation channels of such binaries are known, considerable theoretical uncertainties associated with each channel defeat the robust prediction of how much each channel contributes to the total merger rate density. Given that the time evolution of the merger rate density in some channels is (exactly or nearly) independent of BH masses, clarifying this feature from observational data will shed some light on the nature of BH binaries. On the basis of this motivation, we formulate a methodology to perform a statistical test of whether the mass distribution of BH mergers evolves over time by hypothesis testing. Our statistical test requires neither a priori specification of the mass distribution, which is largely uncertain, nor that of the time dependence of merger rate. We then apply it to mock data for some concrete shapes of the merger rate density and show that the proposed method rejects/(does not reject) the null hypothesis correctly for a large sample size. After this verification, the method is applied to a catalog of the gravitational-wave events obtained during the LIGO-Virgo's third observing run. We find that the selection bias degrades the effectiveness of our method for the O3 catalog owing to the reduction in the number of and the maximum redshifts of the merger events that we can explore. Within the range where the method can be applied, there is no indication of the time evolution of the mass distribution of merger rate density. This limitation will be eased in future observations containing more events, and our hypothesis testing will help determine whether the merger rate density evolves over time independently of BH masses.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


